A Type System for Data Flow and Alias Analysis in ReScript

ReScript is a strongly typed language that targets JavaScript, as an alternative to gradually typed languages, such as TypeScript. In this paper, we present a sound type system for data-flow analysis for a subset of the ReScript language, more specifically for a lambda-calculus with mutability and pattern matching. The type system is a local analysis that collects information about variables that are used at each program point as well as alias information.

==> eptcsdata.tex <==
\providecommand{\firstpage}{116}
\providecommand{\publicationstatus}{M. Marin, L. Leu\c{s}tean (Eds.):\\ 
8th Symposium on Working Formal Methods (FROM 2024)\\
EPTCS 410, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.410.8}{10.4204/EPTCS.410.8}}

